Domain2Vec: Domain Embedding for Unsupervised Domain Adaptation

Conventional unsupervised domain adaptation (UDA) studies the knowledge transfer between a limited number of domains. This neglects the more practical scenario where data are distributed in numerous different domains in the real world. The domain similarity between those domains is critical for domain adaptation performance. To describe and learn relations between different domains, we propose a novel Domain2Vec model to provide vectorial representations of visual domains based on joint learning of feature disentanglement and Gram matrix. To evaluate the effectiveness of our Domain2Vec model, we create two large-scale cross-domain benchmarks. The first one is TinyDA, which contains 54 domains and about one million MNIST-style images. The second benchmark is DomainBank, which is collected from 56 existing vision datasets. We demonstrate that our embedding is capable of predicting domain similarities that match our intuition about visual relations between different domains. Extensive experiments are conducted to demonstrate the power of our new datasets in benchmarking state-of-the-art multi-source domain adaptation methods, as well as the advantage of our proposed model.

==> tables/TinyDA_source_only_cross_domain_result.tex <==
\begin{table*}[]
    \tiny
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Caption}
    \begin{tabular}{}
        
         
    \end{tabular}
    
    \label{table_tiny_da_cross_result}
\end{table*}

==> tables/tiny_da_digit_copy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\caption{Single domain transfer on MNIST, USPS, QMNIST.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{3}{|c|}{}                                                         & \multicolumn{9}{c|}{MNIST}                                                                                                                                                                                                                                                           & \multicolumn{9}{c|}{USPS}                                                                                                                                                                                                                                                            & \multicolumn{9}{c|}{QMNIST}                                                                                                                                                                                                                                                          \\ \cline{4-30} 
\multicolumn{3}{|c|}{}                                                         & \multicolumn{5}{c|}{BSDS500}                                                                                                                                & \multicolumn{4}{c|}{CIFAR10}                                                                                                & \multicolumn{5}{c|}{BSDS500}                                                                                                                                & \multicolumn{4}{c|}{CIFAR10}                                                                                                & \multicolumn{5}{c|}{BSDS500}                                                                                                                                & \multicolumn{4}{c|}{CIFAR10}                                                                                                \\ \cline{4-30} 
\multicolumn{3}{|c|}{\multirow{-3}{*}{}}                                       & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Or}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Or}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Or}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    & {\color[HTML]{3531FF} WB}    & {\color[HTML]{3531FF} BB}    & {\color[HTML]{3531FF} Cr}    & {\color[HTML]{3531FF} GS}    \\ \hline
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{C0C0C0}95.1 & \cellcolor[HTML]{ECF4FF}11.2 & \cellcolor[HTML]{ECF4FF}18.7 & \cellcolor[HTML]{ECF4FF}19.3 & \cellcolor[HTML]{ECF4FF}18.1 & \cellcolor[HTML]{ECF4FF}94.2 & \cellcolor[HTML]{ECF4FF}11.7 & \cellcolor[HTML]{ECF4FF}18.2 & \cellcolor[HTML]{ECF4FF}16.8 & \cellcolor[HTML]{EFEFEF}40.8 & \cellcolor[HTML]{EFEFEF}17.6 & \cellcolor[HTML]{EFEFEF}19.5 & \cellcolor[HTML]{EFEFEF}19.1 & \cellcolor[HTML]{EFEFEF}18.1 & \cellcolor[HTML]{EFEFEF}39.5 & \cellcolor[HTML]{EFEFEF}14.7 & \cellcolor[HTML]{EFEFEF}18.5 & \cellcolor[HTML]{EFEFEF}17.8 & \cellcolor[HTML]{ECF4FF}95.2 & \cellcolor[HTML]{ECF4FF}11.6 & \cellcolor[HTML]{ECF4FF}18.7 & \cellcolor[HTML]{ECF4FF}18.8 & \cellcolor[HTML]{ECF4FF}17.6 & \cellcolor[HTML]{ECF4FF}94.4 & \cellcolor[HTML]{ECF4FF}12.5 & \cellcolor[HTML]{ECF4FF}17.9 & \cellcolor[HTML]{ECF4FF}16.7 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{ECF4FF}12.3 & \cellcolor[HTML]{C0C0C0}97.9 & \cellcolor[HTML]{ECF4FF}98.2 & \cellcolor[HTML]{ECF4FF}28.8 & \cellcolor[HTML]{ECF4FF}26.1 & \cellcolor[HTML]{ECF4FF}10.6 & \cellcolor[HTML]{ECF4FF}97.1 & \cellcolor[HTML]{ECF4FF}22.9 & \cellcolor[HTML]{ECF4FF}21.2 & \cellcolor[HTML]{EFEFEF}11.8 & \cellcolor[HTML]{EFEFEF}44.0 & \cellcolor[HTML]{EFEFEF}47.3 & \cellcolor[HTML]{EFEFEF}21.3 & \cellcolor[HTML]{EFEFEF}20.2 & \cellcolor[HTML]{EFEFEF}10.7 & \cellcolor[HTML]{EFEFEF}40.6 & \cellcolor[HTML]{EFEFEF}17.8 & \cellcolor[HTML]{EFEFEF}16.9 & \cellcolor[HTML]{ECF4FF}12.3 & \cellcolor[HTML]{ECF4FF}97.7 & \cellcolor[HTML]{ECF4FF}98.2 & \cellcolor[HTML]{ECF4FF}28.8 & \cellcolor[HTML]{ECF4FF}26.1 & \cellcolor[HTML]{ECF4FF}11.2 & \cellcolor[HTML]{ECF4FF}97.1 & \cellcolor[HTML]{ECF4FF}22.4 & \cellcolor[HTML]{ECF4FF}21.0 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Or} & \cellcolor[HTML]{ECF4FF}14.9 & \cellcolor[HTML]{ECF4FF}78.5 & \cellcolor[HTML]{C0C0C0}98.5 & \cellcolor[HTML]{ECF4FF}38.8 & \cellcolor[HTML]{ECF4FF}36.9 & \cellcolor[HTML]{ECF4FF}12.5 & \cellcolor[HTML]{ECF4FF}82.0 & \cellcolor[HTML]{ECF4FF}25.7 & \cellcolor[HTML]{ECF4FF}24.7 & \cellcolor[HTML]{EFEFEF}11.5 & \cellcolor[HTML]{EFEFEF}32.5 & \cellcolor[HTML]{EFEFEF}49.5 & \cellcolor[HTML]{EFEFEF}18.0 & \cellcolor[HTML]{EFEFEF}16.9 & \cellcolor[HTML]{EFEFEF}8.6  & \cellcolor[HTML]{EFEFEF}33.9 & \cellcolor[HTML]{EFEFEF}13.3 & \cellcolor[HTML]{EFEFEF}13.0 & \cellcolor[HTML]{ECF4FF}15.5 & \cellcolor[HTML]{ECF4FF}77.7 & \cellcolor[HTML]{FFCCC9}98.5 & \cellcolor[HTML]{ECF4FF}39.0 & \cellcolor[HTML]{ECF4FF}36.4 & \cellcolor[HTML]{ECF4FF}12.4 & \cellcolor[HTML]{ECF4FF}82.4 & \cellcolor[HTML]{ECF4FF}25.6 & \cellcolor[HTML]{ECF4FF}24.4 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{ECF4FF}89.2 & \cellcolor[HTML]{ECF4FF}77.9 & \cellcolor[HTML]{ECF4FF}97.3 & \cellcolor[HTML]{C0C0C0}95.3 & \cellcolor[HTML]{ECF4FF}83.6 & \cellcolor[HTML]{ECF4FF}86.0 & \cellcolor[HTML]{ECF4FF}73.8 & \cellcolor[HTML]{ECF4FF}86.2 & \cellcolor[HTML]{ECF4FF}74.8 & \cellcolor[HTML]{EFEFEF}16.2 & \cellcolor[HTML]{EFEFEF}15.2 & \cellcolor[HTML]{EFEFEF}17.2 & \cellcolor[HTML]{EFEFEF}21.1 & \cellcolor[HTML]{EFEFEF}12.5 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{EFEFEF}12.1 & \cellcolor[HTML]{EFEFEF}15.7 & \cellcolor[HTML]{EFEFEF}11.4 & \cellcolor[HTML]{ECF4FF}89.5 & \cellcolor[HTML]{ECF4FF}77.5 & \cellcolor[HTML]{ECF4FF}97.2 & \cellcolor[HTML]{ECF4FF}95.4 & \cellcolor[HTML]{ECF4FF}83.3 & \cellcolor[HTML]{ECF4FF}86.2 & \cellcolor[HTML]{ECF4FF}73.6 & \cellcolor[HTML]{ECF4FF}86.8 & \cellcolor[HTML]{ECF4FF}74.7 \\ %\cline{3-30} 
                         & \multirow{-5}{*}{\myrotate{BSDS500}}  & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{ECF4FF}86.3 & \cellcolor[HTML]{ECF4FF}88.1 & \cellcolor[HTML]{ECF4FF}97.1 & \cellcolor[HTML]{ECF4FF}78.1 & \cellcolor[HTML]{C0C0C0}87.4 & \cellcolor[HTML]{ECF4FF}84.9 & \cellcolor[HTML]{ECF4FF}87.1 & \cellcolor[HTML]{ECF4FF}69.0 & \cellcolor[HTML]{ECF4FF}76.1 & \cellcolor[HTML]{EFEFEF}18.9 & \cellcolor[HTML]{EFEFEF}14.1 & \cellcolor[HTML]{EFEFEF}14.6 & \cellcolor[HTML]{EFEFEF}11.7 & \cellcolor[HTML]{EFEFEF}11.4 & \cellcolor[HTML]{EFEFEF}17.7 & \cellcolor[HTML]{EFEFEF}14.1 & \cellcolor[HTML]{EFEFEF}9.9  & \cellcolor[HTML]{EFEFEF}11.3 & \cellcolor[HTML]{ECF4FF}86.4 & \cellcolor[HTML]{ECF4FF}88.6 & \cellcolor[HTML]{ECF4FF}97.0 & \cellcolor[HTML]{ECF4FF}77.8 & \cellcolor[HTML]{FFCCC9}87.0 & \cellcolor[HTML]{ECF4FF}85.2 & \cellcolor[HTML]{ECF4FF}86.7 & \cellcolor[HTML]{ECF4FF}69.8 & \cellcolor[HTML]{ECF4FF}76.6 \\ \cline{2-30} 
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{ECF4FF}96.8 & \cellcolor[HTML]{ECF4FF}11.9 & \cellcolor[HTML]{ECF4FF}12.3 & \cellcolor[HTML]{ECF4FF}12.9 & \cellcolor[HTML]{ECF4FF}13.4 & \cellcolor[HTML]{C0C0C0}97.2 & \cellcolor[HTML]{ECF4FF}10.9 & \cellcolor[HTML]{ECF4FF}12.6 & \cellcolor[HTML]{ECF4FF}12.6 & \cellcolor[HTML]{EFEFEF}33.7 & \cellcolor[HTML]{EFEFEF}14.2 & \cellcolor[HTML]{EFEFEF}18.6 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}16.8 & \cellcolor[HTML]{EFEFEF}33.0 & \cellcolor[HTML]{EFEFEF}14.2 & \cellcolor[HTML]{EFEFEF}14.9 & \cellcolor[HTML]{EFEFEF}15.4 & \cellcolor[HTML]{FFCCC9}96.9 & \cellcolor[HTML]{ECF4FF}12.1 & \cellcolor[HTML]{ECF4FF}12.3 & \cellcolor[HTML]{ECF4FF}13.1 & \cellcolor[HTML]{ECF4FF}13.1 & \cellcolor[HTML]{FFCCC9}97.3 & \cellcolor[HTML]{ECF4FF}10.5 & \cellcolor[HTML]{ECF4FF}12.4 & \cellcolor[HTML]{ECF4FF}12.6 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{ECF4FF}14.7 & \cellcolor[HTML]{ECF4FF}97.5 & \cellcolor[HTML]{ECF4FF}97.6 & \cellcolor[HTML]{ECF4FF}21.4 & \cellcolor[HTML]{ECF4FF}20.7 & \cellcolor[HTML]{ECF4FF}12.8 & \cellcolor[HTML]{C0C0C0}97.2 & \cellcolor[HTML]{ECF4FF}17.2 & \cellcolor[HTML]{ECF4FF}17.4 & \cellcolor[HTML]{EFEFEF}18.2 & \cellcolor[HTML]{EFEFEF}39.9 & \cellcolor[HTML]{EFEFEF}46.6 & \cellcolor[HTML]{EFEFEF}17.7 & \cellcolor[HTML]{EFEFEF}17.8 & \cellcolor[HTML]{EFEFEF}18.7 & \cellcolor[HTML]{EFEFEF}38.7 & \cellcolor[HTML]{EFEFEF}15.9 & \cellcolor[HTML]{EFEFEF}16.1 & \cellcolor[HTML]{ECF4FF}14.1 & \cellcolor[HTML]{ECF4FF}97.7 & \cellcolor[HTML]{ECF4FF}97.6 & \cellcolor[HTML]{ECF4FF}20.8 & \cellcolor[HTML]{ECF4FF}20.2 & \cellcolor[HTML]{ECF4FF}12.5 & \cellcolor[HTML]{ECF4FF}97.2 & \cellcolor[HTML]{ECF4FF}17.4 & \cellcolor[HTML]{ECF4FF}17.3 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{ECF4FF}86.4 & \cellcolor[HTML]{ECF4FF}84.6 & \cellcolor[HTML]{ECF4FF}96.8 & \cellcolor[HTML]{ECF4FF}94.3 & \cellcolor[HTML]{ECF4FF}84.2 & \cellcolor[HTML]{ECF4FF}85.9 & \cellcolor[HTML]{ECF4FF}83.9 & \cellcolor[HTML]{C0C0C0}90.8 & \cellcolor[HTML]{ECF4FF}83.6 & \cellcolor[HTML]{EFEFEF}13.0 & \cellcolor[HTML]{EFEFEF}14.0 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{EFEFEF}15.8 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{EFEFEF}11.9 & \cellcolor[HTML]{EFEFEF}14.2 & \cellcolor[HTML]{EFEFEF}15.1 & \cellcolor[HTML]{EFEFEF}11.6 & \cellcolor[HTML]{ECF4FF}87.0 & \cellcolor[HTML]{ECF4FF}84.3 & \cellcolor[HTML]{ECF4FF}96.9 & \cellcolor[HTML]{ECF4FF}94.9 & \cellcolor[HTML]{ECF4FF}83.8 & \cellcolor[HTML]{ECF4FF}85.5 & \cellcolor[HTML]{ECF4FF}84.3 & \cellcolor[HTML]{ECF4FF}91.2 & \cellcolor[HTML]{ECF4FF}83.5 \\ %\cline{3-30} 
\multirow{-9}{*}{\myrotate{MNIST}}  & \multirow{-4}{*}{\myrotate{CIFAR10}} & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{ECF4FF}84.8 & \cellcolor[HTML]{ECF4FF}85.1 & \cellcolor[HTML]{ECF4FF}96.6 & \cellcolor[HTML]{ECF4FF}77.7 & \cellcolor[HTML]{ECF4FF}86.4 & \cellcolor[HTML]{ECF4FF}85.0 & \cellcolor[HTML]{ECF4FF}87.6 & \cellcolor[HTML]{ECF4FF}76.2 & \cellcolor[HTML]{C0C0C0}83.9 & \cellcolor[HTML]{EFEFEF}13.9 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}16.8 & \cellcolor[HTML]{EFEFEF}12.9 & \cellcolor[HTML]{EFEFEF}12.1 & \cellcolor[HTML]{EFEFEF}12.1 & \cellcolor[HTML]{EFEFEF}16.0 & \cellcolor[HTML]{EFEFEF}11.4 & \cellcolor[HTML]{EFEFEF}11.5 & \cellcolor[HTML]{ECF4FF}84.5 & \cellcolor[HTML]{ECF4FF}85.2 & \cellcolor[HTML]{ECF4FF}96.5 & \cellcolor[HTML]{ECF4FF}76.9 & \cellcolor[HTML]{ECF4FF}85.9 & \cellcolor[HTML]{ECF4FF}84.8 & \cellcolor[HTML]{ECF4FF}87.5 & \cellcolor[HTML]{ECF4FF}76.5 & \cellcolor[HTML]{FFCCC9}85.0 \\ \hline
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{EFEFEF}32.9 & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}14.6 & \cellcolor[HTML]{EFEFEF}14.0 & \cellcolor[HTML]{EFEFEF}15.3 & \cellcolor[HTML]{EFEFEF}31.1 & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}13.2 & \cellcolor[HTML]{EFEFEF}12.8 & \cellcolor[HTML]{C0C0C0}89.8 & \cellcolor[HTML]{ECF4FF}17.6 & \cellcolor[HTML]{ECF4FF}9.7  & \cellcolor[HTML]{ECF4FF}24.7 & \cellcolor[HTML]{ECF4FF}22.9 & \cellcolor[HTML]{FFCCC9}86.4 & \cellcolor[HTML]{ECF4FF}10.1 & \cellcolor[HTML]{ECF4FF}23.6 & \cellcolor[HTML]{ECF4FF}22.8 & \cellcolor[HTML]{EFEFEF}33.1 & \cellcolor[HTML]{EFEFEF}13.3 & \cellcolor[HTML]{EFEFEF}14.6 & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}14.9 & \cellcolor[HTML]{EFEFEF}31.3 & \cellcolor[HTML]{EFEFEF}14.3 & \cellcolor[HTML]{EFEFEF}13.2 & \cellcolor[HTML]{EFEFEF}13.1 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{EFEFEF}12.4 & \cellcolor[HTML]{EFEFEF}40.1 & \cellcolor[HTML]{EFEFEF}37.6 & \cellcolor[HTML]{EFEFEF}19.8 & \cellcolor[HTML]{EFEFEF}18.4 & \cellcolor[HTML]{EFEFEF}12.8 & \cellcolor[HTML]{EFEFEF}38.0 & \cellcolor[HTML]{EFEFEF}15.9 & \cellcolor[HTML]{EFEFEF}15.4 & \cellcolor[HTML]{ECF4FF}18.8 & \cellcolor[HTML]{C0C0C0}90.4 & \cellcolor[HTML]{FFCCC9}92.6 & \cellcolor[HTML]{ECF4FF}44.4 & \cellcolor[HTML]{ECF4FF}41.4 & \cellcolor[HTML]{ECF4FF}16.0 & \cellcolor[HTML]{ECF4FF}86.5 & \cellcolor[HTML]{ECF4FF}30.5 & \cellcolor[HTML]{ECF4FF}28.7 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{EFEFEF}39.4 & \cellcolor[HTML]{EFEFEF}37.7 & \cellcolor[HTML]{EFEFEF}19.9 & \cellcolor[HTML]{EFEFEF}18.8 & \cellcolor[HTML]{EFEFEF}12.7 & \cellcolor[HTML]{EFEFEF}37.5 & \cellcolor[HTML]{EFEFEF}15.8 & \cellcolor[HTML]{EFEFEF}15.5 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Or} & \cellcolor[HTML]{EFEFEF}22.1 & \cellcolor[HTML]{EFEFEF}18.4 & \cellcolor[HTML]{EFEFEF}25.9 & \cellcolor[HTML]{EFEFEF}17.3 & \cellcolor[HTML]{EFEFEF}17.3 & \cellcolor[HTML]{EFEFEF}20.3 & \cellcolor[HTML]{EFEFEF}17.9 & \cellcolor[HTML]{EFEFEF}16.4 & \cellcolor[HTML]{EFEFEF}16.4 & \cellcolor[HTML]{ECF4FF}15.4 & \cellcolor[HTML]{ECF4FF}58.0 & \cellcolor[HTML]{C0C0C0}89.2 & \cellcolor[HTML]{ECF4FF}38.0 & \cellcolor[HTML]{ECF4FF}38.3 & \cellcolor[HTML]{ECF4FF}12.6 & \cellcolor[HTML]{ECF4FF}49.2 & \cellcolor[HTML]{ECF4FF}28.4 & \cellcolor[HTML]{ECF4FF}28.4 & \cellcolor[HTML]{EFEFEF}22.4 & \cellcolor[HTML]{EFEFEF}18.5 & \cellcolor[HTML]{EFEFEF}25.9 & \cellcolor[HTML]{EFEFEF}17.3 & \cellcolor[HTML]{EFEFEF}18.1 & \cellcolor[HTML]{EFEFEF}20.2 & \cellcolor[HTML]{EFEFEF}18.0 & \cellcolor[HTML]{EFEFEF}16.0 & \cellcolor[HTML]{EFEFEF}16.3 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{EFEFEF}20.0 & \cellcolor[HTML]{EFEFEF}18.8 & \cellcolor[HTML]{EFEFEF}29.8 & \cellcolor[HTML]{EFEFEF}25.2 & \cellcolor[HTML]{EFEFEF}17.8 & \cellcolor[HTML]{EFEFEF}19.0 & \cellcolor[HTML]{EFEFEF}18.0 & \cellcolor[HTML]{EFEFEF}20.5 & \cellcolor[HTML]{EFEFEF}15.1 & \cellcolor[HTML]{ECF4FF}77.0 & \cellcolor[HTML]{ECF4FF}70.1 & \cellcolor[HTML]{ECF4FF}91.5 & \cellcolor[HTML]{C0C0C0}88.1 & \cellcolor[HTML]{ECF4FF}76.2 & \cellcolor[HTML]{ECF4FF}65.1 & \cellcolor[HTML]{ECF4FF}51.5 & \cellcolor[HTML]{ECF4FF}80.1 & \cellcolor[HTML]{ECF4FF}72.5 & \cellcolor[HTML]{EFEFEF}19.6 & \cellcolor[HTML]{EFEFEF}18.4 & \cellcolor[HTML]{EFEFEF}29.9 & \cellcolor[HTML]{EFEFEF}24.6 & \cellcolor[HTML]{EFEFEF}17.7 & \cellcolor[HTML]{EFEFEF}18.7 & \cellcolor[HTML]{EFEFEF}17.4 & \cellcolor[HTML]{EFEFEF}20.1 & \cellcolor[HTML]{EFEFEF}15.2 \\ %\cline{3-30} 
                         & \multirow{-5}{*}{\myrotate{BSDS500}}  & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}13.3 & \cellcolor[HTML]{EFEFEF}19.9 & \cellcolor[HTML]{EFEFEF}14.8 & \cellcolor[HTML]{EFEFEF}15.7 & \cellcolor[HTML]{EFEFEF}14.2 & \cellcolor[HTML]{EFEFEF}11.8 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{EFEFEF}12.4 & \cellcolor[HTML]{ECF4FF}71.2 & \cellcolor[HTML]{ECF4FF}70.6 & \cellcolor[HTML]{ECF4FF}89.7 & \cellcolor[HTML]{ECF4FF}77.7 & \cellcolor[HTML]{C0C0C0}79.8 & \cellcolor[HTML]{ECF4FF}62.0 & \cellcolor[HTML]{ECF4FF}61.9 & \cellcolor[HTML]{ECF4FF}73.6 & \cellcolor[HTML]{ECF4FF}77.1 & \cellcolor[HTML]{EFEFEF}13.8 & \cellcolor[HTML]{EFEFEF}13.0 & \cellcolor[HTML]{EFEFEF}19.9 & \cellcolor[HTML]{EFEFEF}16.1 & \cellcolor[HTML]{EFEFEF}15.3 & \cellcolor[HTML]{EFEFEF}13.5 & \cellcolor[HTML]{EFEFEF}12.0 & \cellcolor[HTML]{EFEFEF}11.7 & \cellcolor[HTML]{EFEFEF}13.1 \\ \cline{2-30} 
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{EFEFEF}28.1 & \cellcolor[HTML]{EFEFEF}13.0 & \cellcolor[HTML]{EFEFEF}10.3 & \cellcolor[HTML]{EFEFEF}12.5 & \cellcolor[HTML]{EFEFEF}13.1 & \cellcolor[HTML]{EFEFEF}27.8 & \cellcolor[HTML]{EFEFEF}10.5 & \cellcolor[HTML]{EFEFEF}11.3 & \cellcolor[HTML]{EFEFEF}11.5 & \cellcolor[HTML]{ECF4FF}85.1 & \cellcolor[HTML]{ECF4FF}24.9 & \cellcolor[HTML]{ECF4FF}31.2 & \cellcolor[HTML]{ECF4FF}29.6 & \cellcolor[HTML]{ECF4FF}28.1 & \cellcolor[HTML]{C0C0C0}82.0 & \cellcolor[HTML]{ECF4FF}17.3 & \cellcolor[HTML]{ECF4FF}28.2 & \cellcolor[HTML]{ECF4FF}27.4 & \cellcolor[HTML]{EFEFEF}27.0 & \cellcolor[HTML]{EFEFEF}12.8 & \cellcolor[HTML]{EFEFEF}10.4 & \cellcolor[HTML]{EFEFEF}12.3 & \cellcolor[HTML]{EFEFEF}12.7 & \cellcolor[HTML]{EFEFEF}27.7 & \cellcolor[HTML]{EFEFEF}10.6 & \cellcolor[HTML]{EFEFEF}11.4 & \cellcolor[HTML]{EFEFEF}11.4 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{EFEFEF}15.4 & \cellcolor[HTML]{EFEFEF}33.3 & \cellcolor[HTML]{EFEFEF}38.8 & \cellcolor[HTML]{EFEFEF}19.5 & \cellcolor[HTML]{EFEFEF}19.4 & \cellcolor[HTML]{EFEFEF}15.6 & \cellcolor[HTML]{EFEFEF}32.9 & \cellcolor[HTML]{EFEFEF}15.5 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{ECF4FF}18.8 & \cellcolor[HTML]{FFCCC9}90.9 & \cellcolor[HTML]{ECF4FF}91.8 & \cellcolor[HTML]{ECF4FF}36.2 & \cellcolor[HTML]{ECF4FF}35.7 & \cellcolor[HTML]{ECF4FF}16.7 & \cellcolor[HTML]{C0C0C0}88.5 & \cellcolor[HTML]{ECF4FF}25.8 & \cellcolor[HTML]{ECF4FF}25.7 & \cellcolor[HTML]{EFEFEF}15.4 & \cellcolor[HTML]{EFEFEF}33.0 & \cellcolor[HTML]{EFEFEF}38.8 & \cellcolor[HTML]{EFEFEF}19.7 & \cellcolor[HTML]{EFEFEF}19.4 & \cellcolor[HTML]{EFEFEF}15.5 & \cellcolor[HTML]{EFEFEF}33.0 & \cellcolor[HTML]{EFEFEF}15.7 & \cellcolor[HTML]{EFEFEF}15.0 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{EFEFEF}20.7 & \cellcolor[HTML]{EFEFEF}18.6 & \cellcolor[HTML]{EFEFEF}26.5 & \cellcolor[HTML]{EFEFEF}23.1 & \cellcolor[HTML]{EFEFEF}15.2 & \cellcolor[HTML]{EFEFEF}19.1 & \cellcolor[HTML]{EFEFEF}16.8 & \cellcolor[HTML]{EFEFEF}18.9 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{ECF4FF}80.6 & \cellcolor[HTML]{ECF4FF}73.1 & \cellcolor[HTML]{ECF4FF}91.5 & \cellcolor[HTML]{FFCCC9}88.4 & \cellcolor[HTML]{ECF4FF}81.8 & \cellcolor[HTML]{ECF4FF}74.7 & \cellcolor[HTML]{ECF4FF}57.1 & \cellcolor[HTML]{C0C0C0}85.7 & \cellcolor[HTML]{ECF4FF}82.9 & \cellcolor[HTML]{EFEFEF}21.3 & \cellcolor[HTML]{EFEFEF}18.5 & \cellcolor[HTML]{EFEFEF}26.6 & \cellcolor[HTML]{EFEFEF}21.7 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}18.7 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}19.2 & \cellcolor[HTML]{EFEFEF}14.8 \\ %\cline{3-30} 
\multirow{-9}{*}{\myrotate{USPS}}   & \multirow{-4}{*}{\myrotate{CIFAR10}} & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{EFEFEF}17.0 & \cellcolor[HTML]{EFEFEF}12.3 & \cellcolor[HTML]{EFEFEF}18.6 & \cellcolor[HTML]{EFEFEF}14.1 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{EFEFEF}16.0 & \cellcolor[HTML]{EFEFEF}12.9 & \cellcolor[HTML]{EFEFEF}13.5 & \cellcolor[HTML]{EFEFEF}12.1 & \cellcolor[HTML]{ECF4FF}71.4 & \cellcolor[HTML]{ECF4FF}64.5 & \cellcolor[HTML]{ECF4FF}90.0 & \cellcolor[HTML]{ECF4FF}76.6 & \cellcolor[HTML]{FFCCC9}82.9 & \cellcolor[HTML]{ECF4FF}67.7 & \cellcolor[HTML]{ECF4FF}54.5 & \cellcolor[HTML]{ECF4FF}75.7 & \cellcolor[HTML]{C0C0C0}84.1 & \cellcolor[HTML]{EFEFEF}16.8 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{EFEFEF}18.6 & \cellcolor[HTML]{EFEFEF}13.4 & \cellcolor[HTML]{EFEFEF}12.7 & \cellcolor[HTML]{EFEFEF}16.2 & \cellcolor[HTML]{EFEFEF}12.5 & \cellcolor[HTML]{EFEFEF}12.5 & \cellcolor[HTML]{EFEFEF}12.4 \\ \hline
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{ECF4FF}96.4 & \cellcolor[HTML]{ECF4FF}9.9  & \cellcolor[HTML]{ECF4FF}13.2 & \cellcolor[HTML]{ECF4FF}12.0 & \cellcolor[HTML]{ECF4FF}13.0 & \cellcolor[HTML]{ECF4FF}96.0 & \cellcolor[HTML]{ECF4FF}9.3  & \cellcolor[HTML]{ECF4FF}11.6 & \cellcolor[HTML]{ECF4FF}11.9 & \cellcolor[HTML]{EFEFEF}43.3 & \cellcolor[HTML]{EFEFEF}9.3  & \cellcolor[HTML]{EFEFEF}11.5 & \cellcolor[HTML]{EFEFEF}9.9  & \cellcolor[HTML]{EFEFEF}10.9 & \cellcolor[HTML]{EFEFEF}36.7 & \cellcolor[HTML]{EFEFEF}9.3  & \cellcolor[HTML]{EFEFEF}9.8  & \cellcolor[HTML]{EFEFEF}9.9  & \cellcolor[HTML]{C0C0C0}96.8 & \cellcolor[HTML]{ECF4FF}10.0 & \cellcolor[HTML]{ECF4FF}13.2 & \cellcolor[HTML]{ECF4FF}12.1 & \cellcolor[HTML]{ECF4FF}12.9 & \cellcolor[HTML]{ECF4FF}96.1 & \cellcolor[HTML]{ECF4FF}9.2  & \cellcolor[HTML]{ECF4FF}11.6 & \cellcolor[HTML]{ECF4FF}12.0 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{ECF4FF}11.7 & \cellcolor[HTML]{ECF4FF}96.6 & \cellcolor[HTML]{ECF4FF}96.8 & \cellcolor[HTML]{ECF4FF}31.8 & \cellcolor[HTML]{ECF4FF}28.7 & \cellcolor[HTML]{ECF4FF}10.9 & \cellcolor[HTML]{ECF4FF}95.1 & \cellcolor[HTML]{ECF4FF}22.6 & \cellcolor[HTML]{ECF4FF}20.5 & \cellcolor[HTML]{EFEFEF}16.5 & \cellcolor[HTML]{EFEFEF}40.0 & \cellcolor[HTML]{EFEFEF}39.3 & \cellcolor[HTML]{EFEFEF}22.9 & \cellcolor[HTML]{EFEFEF}21.4 & \cellcolor[HTML]{EFEFEF}16.0 & \cellcolor[HTML]{EFEFEF}35.9 & \cellcolor[HTML]{EFEFEF}20.4 & \cellcolor[HTML]{EFEFEF}20.0 & \cellcolor[HTML]{ECF4FF}11.7 & \cellcolor[HTML]{C0C0C0}96.5 & \cellcolor[HTML]{ECF4FF}96.9 & \cellcolor[HTML]{ECF4FF}32.4 & \cellcolor[HTML]{ECF4FF}28.8 & \cellcolor[HTML]{ECF4FF}10.7 & \cellcolor[HTML]{ECF4FF}95.2 & \cellcolor[HTML]{ECF4FF}22.6 & \cellcolor[HTML]{ECF4FF}20.7 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Or} & \cellcolor[HTML]{ECF4FF}9.9  & \cellcolor[HTML]{ECF4FF}65.7 & \cellcolor[HTML]{ECF4FF}98.2 & \cellcolor[HTML]{ECF4FF}36.6 & \cellcolor[HTML]{ECF4FF}35.7 & \cellcolor[HTML]{ECF4FF}10.8 & \cellcolor[HTML]{ECF4FF}72.9 & \cellcolor[HTML]{ECF4FF}25.6 & \cellcolor[HTML]{ECF4FF}24.8 & \cellcolor[HTML]{EFEFEF}10.1 & \cellcolor[HTML]{EFEFEF}32.2 & \cellcolor[HTML]{EFEFEF}51.0 & \cellcolor[HTML]{EFEFEF}24.2 & \cellcolor[HTML]{EFEFEF}23.5 & \cellcolor[HTML]{EFEFEF}10.5 & \cellcolor[HTML]{EFEFEF}38.3 & \cellcolor[HTML]{EFEFEF}18.5 & \cellcolor[HTML]{EFEFEF}19.1 & \cellcolor[HTML]{ECF4FF}9.7  & \cellcolor[HTML]{ECF4FF}66.0 & \cellcolor[HTML]{C0C0C0}98.2 & \cellcolor[HTML]{ECF4FF}36.9 & \cellcolor[HTML]{ECF4FF}35.0 & \cellcolor[HTML]{ECF4FF}10.5 & \cellcolor[HTML]{ECF4FF}73.2 & \cellcolor[HTML]{ECF4FF}25.3 & \cellcolor[HTML]{ECF4FF}25.3 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{ECF4FF}91.1 & \cellcolor[HTML]{ECF4FF}82.5 & \cellcolor[HTML]{ECF4FF}97.2 & \cellcolor[HTML]{FFCCC9}95.6 & \cellcolor[HTML]{ECF4FF}83.6 & \cellcolor[HTML]{ECF4FF}87.3 & \cellcolor[HTML]{ECF4FF}79.3 & \cellcolor[HTML]{ECF4FF}87.1 & \cellcolor[HTML]{ECF4FF}75.4 & \cellcolor[HTML]{EFEFEF}17.8 & \cellcolor[HTML]{EFEFEF}19.2 & \cellcolor[HTML]{EFEFEF}20.1 & \cellcolor[HTML]{EFEFEF}23.9 & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{EFEFEF}15.2 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}12.2 & \cellcolor[HTML]{ECF4FF}90.9 & \cellcolor[HTML]{ECF4FF}81.8 & \cellcolor[HTML]{ECF4FF}97.3 & \cellcolor[HTML]{C0C0C0}95.8 & \cellcolor[HTML]{ECF4FF}83.9 & \cellcolor[HTML]{ECF4FF}87.6 & \cellcolor[HTML]{ECF4FF}78.3 & \cellcolor[HTML]{ECF4FF}86.9 & \cellcolor[HTML]{ECF4FF}75.0 \\ %\cline{3-30} 
                         & \multirow{-5}{*}{\myrotate{BSDS500}}  & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{ECF4FF}84.9 & \cellcolor[HTML]{ECF4FF}81.0 & \cellcolor[HTML]{ECF4FF}95.8 & \cellcolor[HTML]{ECF4FF}81.7 & \cellcolor[HTML]{ECF4FF}86.8 & \cellcolor[HTML]{ECF4FF}84.4 & \cellcolor[HTML]{ECF4FF}81.4 & \cellcolor[HTML]{ECF4FF}71.9 & \cellcolor[HTML]{ECF4FF}75.8 & \cellcolor[HTML]{EFEFEF}14.9 & \cellcolor[HTML]{EFEFEF}16.4 & \cellcolor[HTML]{EFEFEF}17.4 & \cellcolor[HTML]{EFEFEF}9.4  & \cellcolor[HTML]{EFEFEF}12.0 & \cellcolor[HTML]{EFEFEF}13.7 & \cellcolor[HTML]{EFEFEF}14.6 & \cellcolor[HTML]{EFEFEF}10.1 & \cellcolor[HTML]{EFEFEF}11.1 & \cellcolor[HTML]{ECF4FF}84.9 & \cellcolor[HTML]{ECF4FF}81.7 & \cellcolor[HTML]{ECF4FF}95.8 & \cellcolor[HTML]{ECF4FF}80.6 & \cellcolor[HTML]{C0C0C0}86.4 & \cellcolor[HTML]{ECF4FF}84.0 & \cellcolor[HTML]{ECF4FF}81.6 & \cellcolor[HTML]{ECF4FF}72.3 & \cellcolor[HTML]{ECF4FF}76.5 \\ \cline{2-30} 
                         &                         & {\color[HTML]{3531FF} WB} & \cellcolor[HTML]{ECF4FF}96.6 & \cellcolor[HTML]{ECF4FF}11.0 & \cellcolor[HTML]{ECF4FF}21.8 & \cellcolor[HTML]{ECF4FF}14.1 & \cellcolor[HTML]{ECF4FF}13.7 & \cellcolor[HTML]{ECF4FF}96.7 & \cellcolor[HTML]{ECF4FF}11.7 & \cellcolor[HTML]{ECF4FF}13.3 & \cellcolor[HTML]{ECF4FF}13.2 & \cellcolor[HTML]{EFEFEF}35.0 & \cellcolor[HTML]{EFEFEF}18.8 & \cellcolor[HTML]{EFEFEF}16.0 & \cellcolor[HTML]{EFEFEF}18.0 & \cellcolor[HTML]{EFEFEF}18.0 & \cellcolor[HTML]{EFEFEF}35.9 & \cellcolor[HTML]{EFEFEF}16.6 & \cellcolor[HTML]{EFEFEF}17.7 & \cellcolor[HTML]{EFEFEF}17.0 & \cellcolor[HTML]{ECF4FF}96.5 & \cellcolor[HTML]{ECF4FF}10.9 & \cellcolor[HTML]{ECF4FF}21.7 & \cellcolor[HTML]{ECF4FF}14.3 & \cellcolor[HTML]{ECF4FF}14.1 & \cellcolor[HTML]{C0C0C0}96.8 & \cellcolor[HTML]{ECF4FF}11.0 & \cellcolor[HTML]{ECF4FF}13.5 & \cellcolor[HTML]{ECF4FF}12.7 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} BB} & \cellcolor[HTML]{ECF4FF}11.0 & \cellcolor[HTML]{ECF4FF}97.6 & \cellcolor[HTML]{ECF4FF}98.0 & \cellcolor[HTML]{ECF4FF}19.1 & \cellcolor[HTML]{ECF4FF}17.4 & \cellcolor[HTML]{ECF4FF}11.6 & \cellcolor[HTML]{FFCCC9}97.4 & \cellcolor[HTML]{ECF4FF}14.1 & \cellcolor[HTML]{ECF4FF}13.9 & \cellcolor[HTML]{EFEFEF}16.5 & \cellcolor[HTML]{EFEFEF}33.4 & \cellcolor[HTML]{EFEFEF}37.3 & \cellcolor[HTML]{EFEFEF}18.2 & \cellcolor[HTML]{EFEFEF}17.9 & \cellcolor[HTML]{EFEFEF}16.5 & \cellcolor[HTML]{EFEFEF}32.4 & \cellcolor[HTML]{EFEFEF}15.6 & \cellcolor[HTML]{EFEFEF}15.8 & \cellcolor[HTML]{ECF4FF}11.0 & \cellcolor[HTML]{FFCCC9}97.7 & \cellcolor[HTML]{ECF4FF}98.0 & \cellcolor[HTML]{ECF4FF}18.6 & \cellcolor[HTML]{ECF4FF}16.9 & \cellcolor[HTML]{ECF4FF}11.3 & \cellcolor[HTML]{C0C0C0}97.5 & \cellcolor[HTML]{ECF4FF}14.4 & \cellcolor[HTML]{ECF4FF}13.8 \\ %\cline{3-30} 
                         &                         & {\color[HTML]{3531FF} Cr} & \cellcolor[HTML]{ECF4FF}86.0 & \cellcolor[HTML]{ECF4FF}80.8 & \cellcolor[HTML]{ECF4FF}96.8 & \cellcolor[HTML]{ECF4FF}94.2 & \cellcolor[HTML]{ECF4FF}83.9 & \cellcolor[HTML]{ECF4FF}84.4 & \cellcolor[HTML]{ECF4FF}80.0 & \cellcolor[HTML]{FFCCC9}91.0 & \cellcolor[HTML]{ECF4FF}83.5 & \cellcolor[HTML]{EFEFEF}13.1 & \cellcolor[HTML]{EFEFEF}12.8 & \cellcolor[HTML]{EFEFEF}13.5 & \cellcolor[HTML]{EFEFEF}15.0 & \cellcolor[HTML]{EFEFEF}10.2 & \cellcolor[HTML]{EFEFEF}12.1 & \cellcolor[HTML]{EFEFEF}13.0 & \cellcolor[HTML]{EFEFEF}13.3 & \cellcolor[HTML]{EFEFEF}12.0 & \cellcolor[HTML]{ECF4FF}85.9 & \cellcolor[HTML]{ECF4FF}80.0 & \cellcolor[HTML]{ECF4FF}96.7 & \cellcolor[HTML]{ECF4FF}95.0 & \cellcolor[HTML]{ECF4FF}83.8 & \cellcolor[HTML]{ECF4FF}84.2 & \cellcolor[HTML]{ECF4FF}80.2 & \cellcolor[HTML]{C0C0C0}91.3 & \cellcolor[HTML]{ECF4FF}83.6 \\ %\cline{3-30} 
\multirow{-9}{*}{\myrotate{QMNIST}} & \multirow{-4}{*}{\myrotate{CIFAR10}} & {\color[HTML]{3531FF} GS} & \cellcolor[HTML]{ECF4FF}78.0 & \cellcolor[HTML]{ECF4FF}72.9 & \cellcolor[HTML]{ECF4FF}95.7 & \cellcolor[HTML]{ECF4FF}68.2 & \cellcolor[HTML]{ECF4FF}83.8 & \cellcolor[HTML]{ECF4FF}78.9 & \cellcolor[HTML]{ECF4FF}82.6 & \cellcolor[HTML]{ECF4FF}64.5 & \cellcolor[HTML]{ECF4FF}82.5 & \cellcolor[HTML]{EFEFEF}13.8 & \cellcolor[HTML]{EFEFEF}14.3 & \cellcolor[HTML]{EFEFEF}13.9 & \cellcolor[HTML]{EFEFEF}8.7  & \cellcolor[HTML]{EFEFEF}10.9 & \cellcolor[HTML]{EFEFEF}12.6 & \cellcolor[HTML]{EFEFEF}15.6 & \cellcolor[HTML]{EFEFEF}8.3  & \cellcolor[HTML]{EFEFEF}9.3  & \cellcolor[HTML]{ECF4FF}78.2 & \cellcolor[HTML]{ECF4FF}72.2 & \cellcolor[HTML]{ECF4FF}95.6 & \cellcolor[HTML]{ECF4FF}68.2 & \cellcolor[HTML]{ECF4FF}83.7 & \cellcolor[HTML]{ECF4FF}79.1 & \cellcolor[HTML]{ECF4FF}82.5 & \cellcolor[HTML]{ECF4FF}64.4 & \cellcolor[HTML]{C0C0C0}82.8 \\ \hline
\end{tabular}

\end{table*}

==> tables/tiny_da_kmnist.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\makeatletter
\newcommand{\srcsize}{\@setfontsize{\srcsize}{8pt}{8pt}}
\makeatother
% \srcsize{test}

\begin{table*}[]
{\fontfamily{ptm}\selectfont 
\begin{minipage}{0.33\linewidth}
\tiny
\setlength{\tabcolsep}{0.6pt}
\begin{tabular}{|c|c|c|ccccc|cccc|}

% \setlength{\tabcolsep}{2pt}
\hline

\multicolumn{3}{|c|}{}                                  & \multicolumn{9}{c|}{KMNIST}                                                                                                                                                                                                                                                          \\ \cline{4-12} 
\multicolumn{3}{|c|}{}                                  & \multicolumn{5}{c|}{BSDS}                                                                                                                                & \multicolumn{4}{c|}{CIFAR}                                                                                                \\ \cline{4-12} 
\multicolumn{3}{|c|}{\multirow{-3}{*}{}}                & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            &{\color[HTML]{3531FF} Or}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            \\ \hline
                         &                         & {\color[HTML]{3531FF} WB}  & \cellcolor[HTML]{E0E0E0}89.8 & 13.3                         & 12.4                         & 16.8                         & 16.4                         & \cellcolor[HTML]{FFFFFF}88.0 & 12.8                         & 14.9                         & 14.6                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} BB}  & 12.5                         & \cellcolor[HTML]{E0E0E0}94.1 & 94.3                         & 32.9                         & 30.4                         & 11.5                         & \cellcolor[HTML]{FFFFFF}92.6 & 23.3                         & 22.2                         \\ %\cline{3-12} 
                         &                         &{\color[HTML]{3531FF} Or}  & 8.4                          & 56.9                         & \cellcolor[HTML]{E0E0E0}95.4 & 35.2                         & 32.9                         & 9.3                          & 62.6                         & 24.7                         & 23.2                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} Cr}  & 73.4                         & 68.6                         & 89.8                         & \cellcolor[HTML]{E0E0E0}84.2 & 69.1                         & 66.2                         & 66.5                         & 70.9                         & 56.5                         \\ %\cline{3-12} 
                         & \multirow{-5}{*}{\STAB{\rotatebox[origin=c]{90}{BSDS}}}  & {\color[HTML]{3531FF} GS}  & 72.7                         & 64.0                         & 87.9                         & 67.4                         & \cellcolor[HTML]{E0E0E0}74.1 & 68.7                         & 66.7                         & 55.1                         & 59.4                         \\ \cline{2-12} 
                         &                         & {\color[HTML]{3531FF} WB}  & 83.8                         & 17.0                         & 16.2                         & 18.6                         & 18.9                         & \cellcolor[HTML]{E0E0E0}81.2 & 15.1                         & 18.8                         & 18.0                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} BB}  & 13.1                         & 90.0                         & 91.2                         & 26.0                          & 24.1                         & 11.8                         & \cellcolor[HTML]{E0E0E0}88.8 & 18.8                         & 17.9                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} Cr}  & 66.5                         & 65.8                         & 85.3                         & 81.4                         & 68.8                         & 61.6                         & 65.7                         & \cellcolor[HTML]{E0E0E0}76.1 & 65.7                         \\ %\cline{3-12} 
\multirow{-9}{*}{\STAB{\rotatebox[origin=c]{90}{KMNIST}}} & \multirow{-4}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR}}} & {\color[HTML]{3531FF} GS}  & 64.5                         & 60.5                         & 85.8                         & 58.0                          & 70.7                         & 60.8                         & 63.4                         & 56.7                         & \cellcolor[HTML]{E0E0E0}66.8 \\ \hline
\end{tabular}
\end{minipage}
\begin{minipage}{0.33\linewidth}%
\tiny
\setlength{\tabcolsep}{0.6pt}
\begin{tabular}{|c|c|c|ccccc|cccc|}
\hline
\multicolumn{3}{|c|}{}                                  & \multicolumn{9}{c|}{EMNIST}                                                                                                                                                                                                                                                          \\ \cline{4-12} 
\multicolumn{3}{|c|}{}                                  & \multicolumn{5}{c|}{BSDS}                                                                                                                                & \multicolumn{4}{c|}{CIFAR}                                                                                                \\ \cline{4-12} 
\multicolumn{3}{|c|}{\multirow{-3}{*}{}}                & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            &{\color[HTML]{3531FF} Or}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            \\ \hline
                         &                         & {\color[HTML]{3531FF} WB}  & \cellcolor[HTML]{E0E0E0}86.6 & 2.9                          & 2.8                          & 8.1                          & 8.6                          & 83.2                         & 5.1                          & 6.9                          & 7.5                          \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} BB}  & 3.6                          & \cellcolor[HTML]{E0E0E0}87.3 & 88.0                         & 23.4                         & 18.1                         & 4.2                          & \cellcolor[HTML]{FFFFFF}82.8 & 14.9                         & 13.4                         \\ %\cline{3-12} 
                         &                         &{\color[HTML]{3531FF} Or}  & 12.0                         & 31.1                         & \cellcolor[HTML]{E0E0E0}91.3 & 33.4                         & 32.2                         & 11.1                         & 33.6                         & 21.1                         & 21.2                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} Cr}  & 59.1                         & 47.0                         & 85.8                         & \cellcolor[HTML]{E0E0E0}80.0 & 60.8                         & 47.9                         & 42.0                         & 60.0                         & 42.7                         \\ %\cline{3-12} 
                         & \multirow{-5}{*}{\STAB{\rotatebox[origin=c]{90}{BSDS}}}  & {\color[HTML]{3531FF} GS}  & 59.4                         & 46.7                         & 82.5                         & 56.1                         & \cellcolor[HTML]{E0E0E0}65.9 & 52.2                         & 46.8                         & 41.2                         & 44.6                         \\ \cline{2-12} 
                         &                         & {\color[HTML]{3531FF} WB}  & \cellcolor[HTML]{FFFFFF}87.8 & 13.9                         & 4.5                          & 15.3                         & 16.7                         & \cellcolor[HTML]{E0E0E0}86.1 & 12.2                         & 13.0                         & 13.6                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} BB}  & 2.1                          & 85.4                         & 87.1                         & 18.1                         & 17.1                         & 1.9                          & \cellcolor[HTML]{E0E0E0}82.7 & 12.0                         & 12.5                         \\ %\cline{3-12} 
                         &                         & {\color[HTML]{3531FF} Cr}  & 58.2                         & 48.9                         & 83.5                         & 76.1                         & 59.6                         & 48.4                         & 44.7                         & \cellcolor[HTML]{E0E0E0}67.8 & 55.0                         \\ %\cline{3-12} 
\multirow{-9}{*}{\STAB{\rotatebox[origin=c]{90}{EMNIST}}} & \multirow{-4}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR}}} & {\color[HTML]{3531FF} GS}  & 46.6                         & 46.5                         & 81.1                         & 48.1                         & 63.2                         & 43.8                         & 48.8                         & 45.3                         & \cellcolor[HTML]{E0E0E0}57.4 \\ \hline
\end{tabular}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{0.3\linewidth}%
\tiny
\setlength{\tabcolsep}{0.6pt}
\begin{tabular}{|c|c|c|ccccc|cccc|}
\hline
\multicolumn{3}{|c|}{}                                        & \multicolumn{9}{c|}{FashionMNIST}                                                                                                                                                                                                                                                    \\ \cline{4-12} 
\multicolumn{3}{|c|}{}                                        & \multicolumn{5}{c|}{BSDS}                                                                                                                                & \multicolumn{4}{c|}{CIFAR}                                                                                                \\ \cline{4-12} 
\multicolumn{3}{|c|}{\multirow{-3}{*}{}}                      & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            &{\color[HTML]{3531FF} Or}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            & {\color[HTML]{3531FF} WB}                            & {\color[HTML]{3531FF} BB}                            & {\color[HTML]{3531FF} Cr}                            & {\color[HTML]{3531FF} GS}                            \\ \hline
                               &                         & {\color[HTML]{3531FF} WB}  & \cellcolor[HTML]{E0E0E0}83.5 & 16.9                         & 29.9                         & 27.0                         & 25.6                         & 80.7                         & 16.7                         & 27.3                         & 24.9                         \\ %\cline{3-12} 
                               &                         & {\color[HTML]{3531FF} BB}  & 23.6                         & \cellcolor[HTML]{E0E0E0}84.5 & 85.4                         & 38.1                         & 36.6                         & 21.1                         & 81.7                         & 28.9                         & 28.9                         \\ %\cline{3-12} 
                               &                         &{\color[HTML]{3531FF} Or}  & 15.1                         & 53.6                         & \cellcolor[HTML]{E0E0E0}87.0 & 33.0                         & 33.2                         & 14.8                         & 52.2                         & 23.8                         & 25.1                         \\ %\cline{3-12} 
                               &                         & {\color[HTML]{3531FF} Cr}  & 75.6                         & 68.6                         & 85.2                         & \cellcolor[HTML]{E0E0E0}81.6 & 74.4                         & 69.9                         & 54.7                         & 75.6                         & 71.3                         \\ %\cline{3-12} 
                               & \multirow{-5}{*}{\myrotate{BSDS}}  & {\color[HTML]{3531FF} GS}  & 72.3                         & 66.3                         & 83.5                         & 71.5                         & \cellcolor[HTML]{E0E0E0}77.6 & 70.2                         & 61.9                         & 69.5                         & 73.2                         \\ \cline{2-12} 
                               &                         & {\color[HTML]{3531FF} WB}  & 82.9                         & 18.1                         & 27.2                         & 28.5                         & 28.6                         & \cellcolor[HTML]{E0E0E0}81.8 & 17.0                         & 29.6                         & 29.3                         \\ %\cline{3-12} 
                               &                         & {\color[HTML]{3531FF} BB}  & 21.1                         & \cellcolor[HTML]{FFFFFF}84.8 & 86.2                         & 29.1                         & 28.4                         & 18.1                         & \cellcolor[HTML]{E0E0E0}82.3 & 22.1                         & 23.3                         \\ %\cline{3-12} 
                               &                         & {\color[HTML]{3531FF} Cr}  & 75.1                         & 67.9                         & 85.1                         & \cellcolor[HTML]{FFFFFF}82.2 & 75.6                         & 72.4                         & 62.4                         & \cellcolor[HTML]{E0E0E0}78.6 & \cellcolor[HTML]{FFFFFF}76.6 \\ %\cline{3-12} 
\multirow{-9}{*}{\myrotate{FashionMNIST}} & \multirow{-4}{*}{\myrotate{CIFAR}} & {\color[HTML]{3531FF} GS}  & 67.9                         & 61.8                         & 82.2                         & 65.2                         & 77.0                         & 66.3                         & 58.0                         & 68.7                         & \cellcolor[HTML]{E0E0E0}76.3 \\ \hline
\end{tabular}

\end{minipage}
}
\caption{Single domain transfer on KMNIST, EMNIST, FashionMNIST}

\end{table*}
